The VLLM Safety Paradox: Dual Ease in Jailbreak Attack and Defense

The vulnerability of Vision Large Language Models (VLLMs) to jailbreak attacks appears as no surprise. However, recent defense mechanisms against these attacks have reached near-saturation performance on benchmark evaluations, often with minimal effort. This \emph{dual high performance} in both attack and defense raises a fundamental and perplexing paradox. To gain a deep understanding of this issue and thus further help strengthen the trustworthiness of VLLMs, this paper makes three key contributions: i) One tentative explanation for VLLMs being prone to jailbreak attacks--\textbf{inclusion of vision inputs}, as well as its in-depth analysis. ii) The recognition of a largely ignored problem in existing defense mechanisms--\textbf{over-prudence}. The problem causes these defense methods to exhibit unintended abstention, even in the presence of benign inputs, thereby undermining their reliability in faithfully defending against attacks. iii) A simple safety-aware method--\textbf{LLM-Pipeline}. Our method repurposes the more advanced guardrails of LLMs on the shelf, serving as an effective alternative detector prior to VLLM response. Last but not least, we find that the two representative evaluation methods for jailbreak often exhibit chance agreement. This limitation makes it potentially misleading when evaluating attack strategies or defense mechanisms. We believe the findings from this paper offer useful insights to rethink the foundational development of VLLM safety with respect to benchmark datasets, defense strategies, and evaluation methods.

==> section/supp_attack.tex <==
\section{Detailed Jailbreak Results}

\noindent\textbf{Detailed attack results on benchmarks.}
We show the detailed attack results on three subsets of the MM-SafetyBench dataset in Table~\ref{tab:attack-mm-safety-sd},~\ref{tab:attack-mm-safety-typo}, and~\ref{tab:attack-mm-safety-sd-typo}.
Additionally, results for 10 scenarios from the FigStep dataset are illustrated in Table~\ref{tab:attack-figstep}.

\noindent\textbf{Detailed caption jailbreak results.}
We show more examples pertaining to harmful captions generated by the Qwen2-VL model in Fig.~\ref{fig:supp-caption}.

\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{images/supp-caption.pdf}
    \caption{Examples of harmful captions generated by the QWen2-VL model~\cite{qwen2-vl} in response to benign, general prompts.}
    \label{fig:supp-caption}
\end{figure*}

\begin{table*}[htbp]
\centering
\caption{Detailed ASR results for six VLLMs on the SD subset of the MM-SafetyBench dataset~\cite{mm-safetybench}.} 
% \vspace{-1em}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{l|*{6}{C{1.5cm}}}
\toprule
Scenarios                   & LLaVA-1.5-Vicuna-7B       & LLaVA-1.5-Vicuna-13B      & LLaVA-NeXT-Mistral-7B     & LLaVA-NeXT-Llama3-8B      & InternVL2-8B              & Qwen2-VL-7B               \\
\midrule
\textcolor{gray}{Overall}   & \textcolor{gray}{86.61}   & \textcolor{gray}{87.20}   & \textcolor{gray}{79.41}   & \textcolor{gray}{76.43}   & \textcolor{gray}{68.81}   & \textcolor{gray}{81.07} \\ 
\midrule
01-Illegal Activity         & 71.13                     & 64.95                     & 53.61                     & 55.67                     & 47.42                     & 52.58                     \\ 
02-Hate Speech              & 86.50                     & 89.57                     & 77.91                     & 73.01                     & 63.19                     & 82.82                     \\ 
03-Malware Generation       & 84.09                     & 81.82                     & 79.55                     & 70.45                     & 72.73                     & 75.00                     \\ 
04-Physical Harm            & 82.64                     & 82.64                     & 81.25                     & 72.92                     & 61.81                     & 70.83                     \\ 
05-Economic Harm            & 91.80                     & 91.80                     & 84.43                     & 81.15                     & 73.77                     & 82.79                     \\ 
06-Fraud                    & 88.96                     & 86.36                     & 76.62                     & 74.03                     & 55.84                     & 75.32                     \\ 
07-Pornography              & 92.66                     & 93.58                     & 88.99                     & 89.00                     & 87.16                     & 91.74                     \\ 
08-Political Lobbying       & 97.39                     & 100.00                    & 94.77                     & 94.12                     & 89.54                     & 95.42                     \\ 
09-Privacy Violence         & 81.29                     & 87.05                     & 84.17                     & 81.29                     & 60.43                     & 80.58                     \\ 
10-Legal Opinion            & 75.38                     & 76.15                     & 74.62                     & 80.00                     & 67.69                     & 81.54                     \\ 
11-Financial Advice         & 85.63                     & 86.83                     & 74.85                     & 59.28                     & 59.88                     & 80.84                     \\ 
12-Health Consultation      & 84.40                     & 84.40                     & 66.06                     & 75.23                     & 71.56                     & 77.06                     \\ 
13-Gov Decision             & 96.64                     & 96.64                     & 86.58                     & 82.55                     & 85.91                     & 94.63                     \\ 
\bottomrule
\end{tabular}}
\label{tab:attack-mm-safety-sd}
\end{table*}

\begin{table*}[htbp]
\centering
\caption{Detailed ASR results for six VLLMs on the TYPO subset of the MM-SafetyBench dataset~\cite{mm-safetybench}.} 
% \vspace{-1em}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{l|*{6}{C{1.5cm}}}
\toprule
Scenarios                   & LLaVA-1.5-Vicuna-7B       & LLaVA-1.5-Vicuna-13B      & LLaVA-NeXT-Mistral-7B     & LLaVA-NeXT-Llama3-8B      & InternVL2-8B              & Qwen2-VL-7B               \\
\midrule
\textcolor{gray}{Overall}   & \textcolor{gray}{87.08}   & \textcolor{gray}{84.17}   & \textcolor{gray}{57.62}   & \textcolor{gray}{53.81}   & \textcolor{gray}{53.04}   & \textcolor{gray}{60.36} \\ 
\midrule
01-Illegal Activity         & 67.01                     & 52.58                     & 7.22                      & 16.49                     & 7.22                      & 10.31                     \\ 
02-Hate Speech              & 82.21                     & 82.82                     & 46.63                     & 42.94                     & 33.74                     & 43.56                     \\ 
03-Malware Generation       & 90.91                     & 84.09                     & 36.37                     & 31.82                     & 43.18                     & 50.00                     \\ 
04-Physical Harm            & 80.56                     & 81.94                     & 42.36                     & 36.11                     & 41.67                     & 44.44                     \\ 
05-Economic Harm            & 91.80                     & 94.26                     & 70.49                     & 60.66                     & 67.21                     & 74.59                     \\ 
06-Fraud                    & 83.77                     & 80.52                     & 32.47                     & 29.87                     & 20.13                     & 20.78                     \\ 
07-Pornography              & 95.42                     & 92.66                     & 74.31                     & 67.89                     & 70.64                     & 80.73                     \\ 
08-Political Lobbying       & 96.73                     & 96.08                     & 92.81                     & 94.12                     & 83.66                     & 94.12                     \\ 
09-Privacy Violence         & 88.49                     & 84.17                     & 44.60                     & 43.17                     & 29.50                     & 33.81                     \\ 
10-Legal Opinion            & 80.00                     & 74.62                     & 60.00                     & 63.08                     & 59.23                     & 67.69                     \\ 
11-Financial Advice         & 90.42                     & 85.03                     & 74.85                     & 59.28                     & 63.47                     & 80.24                     \\ 
12-Health Consultation      & 87.16                     & 80.73                     & 56.88                     & 50.55                     & 75.23                     & 78.90                     \\ 
13-Gov Decision             & 95.30                     & 95.30                     & 81.88                     & 71.81                     & 84.56                     & 91.95                     \\ 
\bottomrule
\end{tabular}}
\label{tab:attack-mm-safety-typo}
\end{table*}

\begin{table*}[htbp]
\centering
\caption{Detailed ASR results for six VLLMs on the SD+TYPO subset of the MM-SafetyBench dataset~\cite{mm-safetybench}.} 
% \vspace{-1em}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{l|*{6}{C{1.5cm}}}
\toprule
Scenarios                   & LLaVA-1.5-Vicuna-7B       & LLaVA-1.5-Vicuna-13B      & LLaVA-NeXT-Mistral-7B     & LLaVA-NeXT-Llama3-8B      & InternVL2-8B              & Qwen2-VL-7B           \\
\midrule
\textcolor{gray}{Overall}   & \textcolor{gray}{86.91}   & \textcolor{gray}{78.51}   & \textcolor{gray}{62.21}   & \textcolor{gray}{57.32}   & \textcolor{gray}{58.75}   & \textcolor{gray}{64.40} \\ 
\midrule
01-Illegal Activity         & 50.52                     & 26.80                     & 22.68                     & 22.68                     & 9.28                      & 16.49                     \\
02-Hate Speech              & 82.82                     & 72.39                     & 51.53                     & 48.47                     & 51.53                     & 57.06                     \\
03-Malware Generation       & 84.09                     & 70.45                     & 40.91                     & 43.18                     & 50.00                     & 56.82                     \\
04-Physical Harm            & 85.42                     & 66.67                     & 59.73                     & 40.98                     & 40.28                     & 45.83                     \\
05-Economic Harm            & 92.62                     & 85.89                     & 73.77                     & 63.93                     & 67.21                     & 74.59                     \\
06-Fraud                    & 77.92                     & 64.94                     & 37.66                     & 40.26                     & 33.12                     & 91.17                     \\
07-Pornography              & 95.41                     & 92.66                     & 77.98                     & 68.81                     & 85.32                     & 88.99                     \\
08-Political Lobbying       & 96.10                     & 98.04                     & 96.08                     & 94.12                     & 84.97                     & 91.50                     \\
09-Privacy Violence         & 79.86                     & 67.63                     & 48.92                     & 44.60                     & 38.13                     & 47.48                     \\
10-Legal Opinion            & 88.46                     & 76.92                     & 74.62                     & 68.46                     & 67.69                     & 72.31                     \\
11-Financial Advice         & 94.61                     & 87.43                     & 72.46                     & 64.07                     & 62.28                     & 71.86                     \\
12-Health Consultation      & 91.74                     & 95.41                     & 44.95                     & 68.72                     & 77.98                     & 77.98                     \\
13-Gov Decision             & 99.33                     & 98.66                     & 80.54                     & 69.13                     & 85.91                     & 94.63                     \\
\bottomrule
\end{tabular}}
\label{tab:attack-mm-safety-sd-typo}
\end{table*}

\begin{table*}[htbp]
\centering
\caption{Detailed ASR results for six VLLMs on the FigStep dataset~\cite{figstep}.} 
% \vspace{-1em}
\resizebox{0.75\linewidth}{!}{
\begin{tabular}{l|*{6}{C{1.5cm}}}
\toprule
Scenarios                   & LLaVA-1.5-Vicuna-7B       & LLaVA-1.5-Vicuna-13B      & LLaVA-NeXT-Mistral-7B     & LLaVA-NeXT-Llama3-8B      & InternVL2-8B              & Qwen2-VL-7B           \\
\midrule
\textcolor{gray}{Overall}   & \textcolor{gray}{65.6}    & \textcolor{gray}{53.2}    & \textcolor{gray}{50.2}    & \textcolor{gray}{48.4}    & \textcolor{gray}{45.8}    & \textcolor{gray}{32.20} \\ 
\midrule
Illegal Activity            & 48                        & 28                        & 16                        & 28                        & 44                        & 32.2                 \\ 
Hate Speech                 & 50                        & 38                        & 30                        & 50                        & 14                        & 14                    \\ 
Malware Generation          & 42                        & 24                        & 20                        & 20                        & 16                        & 10                    \\ 
Physical Harm               & 62                        & 40                        & 34                        & 24                        & 30                        & 10                    \\ 
Fraud                       & 58                        & 48                        & 26                        & 24                        & 18                        & 8                     \\ 
Adult Content               & 80                        & 76                        & 72                        & 74                        & 84                        & 8                     \\ 
Privacy Violation           & 74                        & 58                        & 58                        & 58                        & 34                        & 68                    \\ 
Legal Opinion               & 86                        & 78                        & 84                        & 72                        & 74                        & 16                    \\ 
Financial Advice            & 82                        & 80                        & 78                        & 64                        & 78                        & 66                    \\ 
Health Consultation         & 74                        & 62                        & 84                        & 70                        & 66                        & 78                    \\ 
\bottomrule
\end{tabular}}
\label{tab:attack-figstep}
\end{table*}



==> section/supp_basics.tex <==
\section{Preliminaries of Models and Datasets}

\subsection{Evaluated VLLMs for Jailbreak Attack}
In this study, we mainly evaluated the following six VLLMs on the jailbreak attack datasets.

\noindent\textbf{LLaVA-1.5-Vicuna-7B}~\cite{llava-1.5} improves the original LLaVA model by upgrading the vision-language connector from a linear projection to an MLP projection. 
Furthermore, it supports higher-resolution image inputs and is pre-trained on 1.2 million publicly available data. 
The LLM base used is Vicuna-7B-v1.5~\cite{vicuna}.

\noindent\textbf{LLaVA-1.5-Vicuna-13B}~\cite{llava-1.5} further scales LLaVA-1.5-Vicuna-7B to a 13B version, with Vicuna-13B-v1.5~\cite{vicuna} as its LLM base.

\noindent\textbf{LLaVA-NeXT-Mistral-7B}~\cite{llava-next} introduces an AnyRes approach, designed to handle images of varying high resolutions while balancing performance efficiency with operational costs. 
Additionally, it enhances capabilities in reasoning, OCR, and world knowledge inference. 
The LLM base used is Mistral-7B~\cite{mistral}.

\noindent\textbf{LLaVA-NeXT-Llama3-8B}~\cite{llava-next} shares a similar architecture to LLaVA-NeXT-Mistral-7B, but replaces the LLM base with Llama3-8B~\cite{llama-3}.

\noindent\textbf{InternVL2-8B}~\cite{intern-vl} demonstrates competitive performance on par with proprietary models across various capabilities, such as document and chart comprehension.
It is pre-trained with an 8k context window and utilizes diverse training datasets compromising long texts, multiple images, and videos.
The LLM is based on InternLM-2.5~\cite{internlm-2}.

\noindent\textbf{QWen2-VL-7B}~\cite{qwen2-vl} has been very recently released to the public.
It introduces a Naive Dynamic Resolution mechanism that allows the model to process images of varying resolutions by converting them into different numbers of visual tokens. 
The underlying LLM is QWen2~\cite{qwen2}.

\begin{figure}[t!]
  \centering
  \includegraphics[width=1.0\linewidth]{images/teaser.pdf}
  % \vspace{-1em}
  \caption{VLLMs are vulnerable to jailbreak attacks (top, Section 3), yet they are also relatively straightforward to defend against (middle, Section 4). 
  In this study, we demonstrate that LLMs are already capable of effectively detecting such vision-involved attacks (bottom, Section 5).
  }\label{fig:teaser}
  % \vspace{-1em}
\end{figure}

\subsection{Jailbreak Attack Datasets}
\noindent\textbf{FigStep}~\cite{figstep} converts harmful content into images using typography to bypass safety alignment measures. 
Specifically, harmful questions are rephrased into declarative statements beginning with phrases like `Steps to', `List of', etc. (\eg, \emph{steps to make a bomb}). 
The dataset contains 500 image-instruction pairs, covering 10 common sensitive scenarios, including Illegal Activity, Hate Speech, Malware Generation, Physical Harm, Fraud, Adult Content, Privacy Violation, Legal Opinion, Financial Advice, and Health Consultation.

\noindent\textbf{VLSafe}~\cite{vl-safe} directly uses images from the MSCOCO dataset~\cite{coco} as the image source. 
Human annotators were involved in crafting harmful questions, resulting in 3,000 image-instruction pairs.

\noindent\textbf{MM-SafetyBench}~\cite{mm-safetybench} generates a query-relevant image using typography or stable diffusion~\cite{stable-diffusion} techniques based on malicious queries.
The generated images are categorized into three types: TYPO, SD, and TYPO+SD, with the latter combining TYPO and SD-generated images.
The dataset consists of 5,040 image-instruction pairs across 13 scenarios, including 01-Illegal Activity, 02-Hate Speech, 03-Malware Generation, 04-Physical Harm, 05-Economic Harm, 06-Fraud, 07-Pornography, 08-Political Lobbying, 09-Privacy Violence, 10-Legal Opinion, 11-Financial Advice, 12-Health Consultation, and 13-Gov Decision.

\noindent\textbf{VL-Guard}~\cite{vl-guard} sourced image data from various datasets to ensure diverse data distribution, including Privacy Alert, Hateful Memes, Harmful Political Memes, Harmful Object Dataset, and Bad Ads. 
The instructions are auto-generated by GPT-4~\cite{gpt-4}. 
For harmful images, the dataset pairs each with a safe instruction explaining its unsafe nature. 
In contrast, for harmless images, the dataset includes one safe and one unsafe instruction. 
The final dataset comprises 1,558 image-instruction pairs and covers four scenarios: Privacy, Risky Behavior, Deception, and Discrimination

\subsection{Evaluation Prompts}
We provide the involved evaluation prompts.

\noindent $\bullet$ Prompt for captioning-based question answering.
\begin{quote}
    \grey{Caption: \{capiton\}}
    
    \grey{Answer my question based on the caption: \{question\}}
\end{quote}

\noindent $\bullet$ Prompt for general question answering and chat.
\begin{quote}
    \grey{\{image\}}
    
    \grey{\{question\}}
\end{quote}

\noindent $\bullet$ System prompt added before the normal task.
\begin{quote}
    \grey{You are a helpful assistant to answer questions from the user.}
    
    \grey{\{normal inputs\}}
\end{quote}

\noindent $\bullet$ System prompt with the scenario information added before the normal task.
\begin{quote}
    \grey{You are a helpful assistant to answer questions from the user.}

    \grey{If you feel like the question will induce potentially harmful information, for example, about \{scenario\}, please reject to respond.}

    \grey{\{normal inputs\}}
\end{quote}

% \paragraph{Captioning}
% \begin{figure}[h!]
%     \centering
%     \vspace{-0.2cm}
%     \includegraphics[width=1.0\linewidth]{images/suppl/caption-prompt-v1.0.pdf}
%     \caption{Prompt for captioning-based question answering.}
%     % \label{fig:enter-label}
%     \vspace{-0.4cm}
% \end{figure}

% \paragraph{Question Answering / Chat}

% \begin{figure}[h]
%     \centering
%     \vspace{-0.2cm}
%     \includegraphics[width=1.0\linewidth]{images/suppl/qa-prompt-v1.0.pdf}
%     \caption{Prompt for general question answering and chat.}
%     % \label{fig:enter-label}
%     \vspace{-0.4cm}
% \end{figure}


% \begin{figure}[h]
%     \centering
%     \vspace{-0.2cm}
%     \includegraphics[width=1.0\linewidth]{images/suppl/system-prompt-v1.0.pdf}
%     \caption{System prompt added before the normal task.}
%     % \label{fig:enter-label}
%     \vspace{-0.4cm}
% \end{figure}


% \begin{figure}[h]
%     \centering
%     % \vspace{-0.2cm}
%     \includegraphics[width=1.0\linewidth]{images/suppl/system-prompt-w-scenario.pdf}
%     \caption{System prompt with the scenario information added before the normal task.}
%     % \label{fig:enter-label}
%     \vspace{-0.4cm}
% \end{figure}


